A Feature Analysis for Multimodal News Retrieval

Content-based information retrieval is based on the information contained in documents rather than using metadata such as keywords. Most information retrieval methods are either based on text or image. In this paper, we investigate the usefulness of multimodal features for cross-lingual news search in various domains: politics, health, environment, sport, and finance. To this end, we consider five feature types for image and text and compare the performance of the retrieval system using different combinations. Experimental results show that retrieval results can be improved when considering both visual and textual information. In addition, it is observed that among textual features entity overlap outperforms word embeddings, while geolocation embeddings achieve better performance among visual features in the retrieval task.

==> Cleopatra Workshop 2020 - Multimodal Feature Analysis for Information Retrieval in News/multirow/README <==
multirow.sty  2019/05/31 v2.5
bigstruts.sty  2019/05/31 v2.5
bigdelim.sty  2019/05/31 v2.5

Original Author: Jerry Leichter
Current Author:  Piet van Oostrum <piet@vanoostrum.org>

 This file may be distributed under the terms of the LaTeX Project Public
 License, as described in lppl.txt in the base LaTeX distribution.
 Either version 1.3 or, at your option, any later version.

Installation:

To generate the .sty files, run the command
   tex multirow.ins
and move the resulting .sty files to a place where LaTeX can find them, preferably
..../tex/latex/multirow

Usage:

multirow.sty:

Make an entry that will span multiple rows of a table.

\multirow[vpos]{nrows}[bigstruts]{width}[vmove]{text}

vpos is the vertical positioning: t. c. or b.

nrows is the number of rows to span.  It's up to you to leave the other
      rows empty, or the stuff created by \multirow will over-write it.
      With a positive value of nrows the spanned colomns are this row and
      (nrows-1) rows below it. With a negative value of nrows they are
      this row and (1-nrows) above it.

bigstruts is mainly used if you've used bigstrut.sty.  In that case it
      is the total number of uses of \bigstrut within the rows being
      spanned.  Count 2 uses for each \bigstrut, 1 for each \bigstrut[x]
      where x is either t or b.  The default is 0.

width is the width to which the text is to be set, or * to indicate that
      the text argument's natural width is to be used.
text is the actual text.  If the width was set explicitly, the text will
      be set in a parbox of that width; you can use \\ to force linebreaks
      where you like.

      If the width was given as * the text will be set in LR mode.  If you
      want a multiline entry in this case you should use a tabular or array
      in the text parameter.

	  If the width is given as = the width will be taken from the
	  tabular column in which it appears. This only works for p{}
	  columns and similar, for example X columns in tabularx, and LCRJ
	  columns in tabulary.

      The text is centered vertically within the range spanned by nrows,
	  unless a vpos argument is given.

vmove is a length used for fine tuning:  The text will be raised (or
      lowered, if vmove is negative) by that length above (below) wherever
       it would otherwise have gone.

For example (using both multirow and bigstrut)

\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}
\begin{tabular}{|c|c|}
\hline
\multirow{4}{1in}{Common g text} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\multirow{3}[6]*{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\
\hline
\multirow{4}[8]{1in}{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\\cline{2-2}
      & Column g2d \bigstrut\\
\hline
\multirow{4}*{\minitab[c]{Common \\ g text}} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\end{tabular}

If any of the spanned rows are unusually large, or if you're using
bigstrut.sty and \bigstrut's are used assymetrically about the centerline of
the spanned rows, the vertical centering may not come out right.  Use the
vmove argument in this case.

Just before "text" is expanded, the \multirowsetup macro is expanded to      
set up any special environment.  Initially, \multirowsetup contains just
\raggedright.  It can be redefined with \renewcommand.
 
bigstrut.sty:

\bigstrut[pos] where pos is t or b

    Add a bit of space above, below, or both a tabular row. The amount
	is determined by \bigstrutjot.

bigdelim.sty:

\ldelim({n}{width}[text]
\rdelim){n}{width}[text]

Put a big delimiter over n rows in a tabular, optionally preceded
(\ldelim) or followed (rdelim) by text.
	


==> multirow/README <==
multirow.sty  2019/05/31 v2.5
bigstruts.sty  2019/05/31 v2.5
bigdelim.sty  2019/05/31 v2.5

Original Author: Jerry Leichter
Current Author:  Piet van Oostrum <piet@vanoostrum.org>

 This file may be distributed under the terms of the LaTeX Project Public
 License, as described in lppl.txt in the base LaTeX distribution.
 Either version 1.3 or, at your option, any later version.

Installation:

To generate the .sty files, run the command
   tex multirow.ins
and move the resulting .sty files to a place where LaTeX can find them, preferably
..../tex/latex/multirow

Usage:

multirow.sty:

Make an entry that will span multiple rows of a table.

\multirow[vpos]{nrows}[bigstruts]{width}[vmove]{text}

vpos is the vertical positioning: t. c. or b.

nrows is the number of rows to span.  It's up to you to leave the other
      rows empty, or the stuff created by \multirow will over-write it.
      With a positive value of nrows the spanned colomns are this row and
      (nrows-1) rows below it. With a negative value of nrows they are
      this row and (1-nrows) above it.

bigstruts is mainly used if you've used bigstrut.sty.  In that case it
      is the total number of uses of \bigstrut within the rows being
      spanned.  Count 2 uses for each \bigstrut, 1 for each \bigstrut[x]
      where x is either t or b.  The default is 0.

width is the width to which the text is to be set, or * to indicate that
      the text argument's natural width is to be used.
text is the actual text.  If the width was set explicitly, the text will
      be set in a parbox of that width; you can use \\ to force linebreaks
      where you like.

      If the width was given as * the text will be set in LR mode.  If you
      want a multiline entry in this case you should use a tabular or array
      in the text parameter.

	  If the width is given as = the width will be taken from the
	  tabular column in which it appears. This only works for p{}
	  columns and similar, for example X columns in tabularx, and LCRJ
	  columns in tabulary.

      The text is centered vertically within the range spanned by nrows,
	  unless a vpos argument is given.

vmove is a length used for fine tuning:  The text will be raised (or
      lowered, if vmove is negative) by that length above (below) wherever
       it would otherwise have gone.

For example (using both multirow and bigstrut)

\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}
\begin{tabular}{|c|c|}
\hline
\multirow{4}{1in}{Common g text} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\multirow{3}[6]*{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\
\hline
\multirow{4}[8]{1in}{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\\cline{2-2}
      & Column g2d \bigstrut\\
\hline
\multirow{4}*{\minitab[c]{Common \\ g text}} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\end{tabular}

If any of the spanned rows are unusually large, or if you're using
bigstrut.sty and \bigstrut's are used assymetrically about the centerline of
the spanned rows, the vertical centering may not come out right.  Use the
vmove argument in this case.

Just before "text" is expanded, the \multirowsetup macro is expanded to      
set up any special environment.  Initially, \multirowsetup contains just
\raggedright.  It can be redefined with \renewcommand.
 
bigstrut.sty:

\bigstrut[pos] where pos is t or b

    Add a bit of space above, below, or both a tabular row. The amount
	is determined by \bigstrutjot.

bigdelim.sty:

\ldelim({n}{width}[text]
\rdelim){n}{width}[text]

Put a big delimiter over n rows in a tabular, optionally preceded
(\ldelim) or followed (rdelim) by text.
	

